Local well-posedness result for a class of non-local quasi-linear systems and its application to the justification of Whitham-Boussinesq systems

In this paper we prove a local well-posedness result for a class of quasi-linear systems of hyperbolic type involving Fourier multipliers. Among the physically relevant systems in this class is a family of Whitham-Boussinesq systems arising in the modeling free-surface water waves. Our result allows to prove the rigorous justification of these systems as approximations to the general water waves system on a relevant time scale, independent of the shallowness parameter.

==> ExistenceOfAWeakSolution.tex <==
Let $t_0 > d/2$. We study here the well-posedness in $X^0(\mathbb{R}^d)$ of the linearized Whitham-Boussinesq system around a state $\underline{U} \in W^{1,\infty}([0,T/\epsilon],X^{t_0}(\mathbb{R}^d))\cap L^{\infty}([0,T/\epsilon],X^{t_0+1}(\mathbb{R}^d))$, i.e. 
\begin{align}\label{system linearized around underline U}
        \partial_t U + \sum\limits_{j=1}^d A_j(\underline{U})[\partial_j U] = \epsilon R,
\end{align}
where $A_j(\underline{U})$ is defined by \eqref{A_j}.

The latter equation is to be taken in the sense of distributions.

\begin{mythm}\label{Uniqueness}
    Let $R \in L^1([0,T/\epsilon],X^0(\mathbb{R}^d))$ and suppose that $U \in L^2([0,T/\epsilon],X^0(\mathbb{R}^d))$ satisfies the linearized system \eqref{system linearized around underline U} with $U_0 = U|_{t=0} \in X^0(\mathbb{R}^d)$. Then $U \in C^0([0,T/\epsilon],X^0(\mathbb{R}^d))$. 
\end{mythm}
Before the proof of this theorem, we introduce the regularized version of system \eqref{system linearized around underline U}. 

Let $J_{\alpha} = (1-\alpha\Delta)^{-1/2}$ a regularizing Fourier multiplier of order $-1$. For any $s \geq 0$, the family $\{ J_{\alpha}, \alpha \in ]0,1] \}$ is uniformly bounded in $X^s(\mathbb{R}^d)$, and for all $v \in X^s(\mathbb{R}^d), J_{\alpha}v \to v$ in $X^s(\mathbb{R}^d)$ as $\alpha \to 0$.

\begin{mylem}
    If $U \in L^2([0,T/\epsilon],X^0(\mathbb{R}^d))$ satisfies the linearized system \eqref{system linearized around underline U} with $R \in L^1([0,T/\epsilon],X^0(\mathbb{R}^d))$, then there exists $R_{(\alpha)} \in L^1([0,T/\epsilon],X^0(\mathbb{R}^d))$ such that
    \begin{align}\label{regularized linearized WB system}
        \partial_t J_{\alpha}U + \sum\limits_{j=1}^d A_j(\underline{U})[\partial_j J_{\alpha}U] = \epsilon R_{(\alpha)}.
    \end{align}
\end{mylem}
\begin{proof}
    Applying $J_{\alpha}$ to the system \eqref{system linearized around underline U}, we get
    \begin{align*}
        \partial_t J_{\alpha}U + \sum\limits_{j=1}^d A_j(\underline{U})[\partial_j J_{\alpha}U] = \epsilon J_{\alpha}R - \sum\limits_{j=1}^d [J_{\alpha},A_j(\underline{U})][\partial_j U].
    \end{align*}
    We denote $R_{(\alpha)} = J_{\alpha} - \frac{1}{\epsilon}\sum\limits_{j=1}^d [J_{\alpha},A_j(\underline{U})][\partial_j U]$. We easily see that $R_{(\alpha)} \in L^1([0,T/\epsilon],X^0(\mathbb{R}^d))$ using the same argument as for the proof of Lemma \ref{Lemma energy estimates of order s WB}.
    
    Moreover, using the density of $X^1(\mathbb{R}^d)$ in $X^0(\mathbb{R}^d)$, we get 
    \begin{align*}
        [J_{\alpha},A_j(\underline{U})][\partial_j U] \to 0 \ \ \rm{in} \ \ X^0(\mathbb{R}^d),
    \end{align*}
    and 
    \begin{align*}
        \int_{0,T} |[J_{\alpha},A_j(\underline{U})][\partial_j U]|_{L^2} \rm{dt} \to 0,
    \end{align*}
    as $\alpha \to 0$.
\end{proof}

We now prove Theorem \ref{Uniqueness}.
\begin{proof}
    Thanks to the previous lemma and the Cauchy-Lipschitz theorem, $U$ is in $C^0([0,T/\epsilon],X^0(\mathbb{R}^d))$, so $J_{\alpha}U$ is in $C^0([0,T/\epsilon],X^1(\mathbb{R}^d))$.
    Using the energy estimates of order 0 \eqref{energy estimates of order 0} on $J_{\alpha}U - J_{\alpha'}U$ we get that $(J_{\alpha}U)_{\alpha \geq 0}$ is a Cauchy sequence in $C^0([0,T/\epsilon],X^0(\mathbb{R}^d)$ as $\alpha \to 0$. So $J_{\alpha}U$ converges in $C^0([0,T/\epsilon],X^0(\mathbb{R}^d)$. But $J_{\alpha}U$ converges to $U$ in $L^2([0,T/\epsilon],X^0(\mathbb{R}^d)$. Thus $J_{\alpha}U \to U$ in $C^0([0,T/\epsilon],X^0(\mathbb{R}^d)$ as $\alpha \to 0$.
    
    Using again the energy estimates of order 0 \eqref{energy estimates of order 0} but this time on $J_{\alpha}U$ and passing to the limit $\alpha \to 0$, we get that $U$ satisfies the energy estimates of order $0$ and is thus in $C^0([0,T/\epsilon],X^0(\mathbb{R}^d)$.
\end{proof}

As a direct consequence of Theorem \ref{Uniqueness} we get the following corollary.

\begin{mycoro}
    If $u \in L^2([0,T/\epsilon],X^0(\mathbb{R}^d))$ satisfies the linearized system \eqref{system linearized around underline U} with $R = 0$ and $U_0 = 0$, then $U = 0$. 
\end{mycoro}

This corollary gives the uniqueness of a solution of the Cauchy problem associated with the system \eqref{system linearized around underline U}. We study now the existence of a solution of the latter system associated with an initial condition in $X^0(\mathbb{R}^d)$. 

\begin{mythm}
    For $R \in L^1([0,T/\epsilon],X^0(\mathbb{R}^d)$ and $U_0 \in X^0(\mathbb{R}^d)$, the Cauchy problem associated with the linearized system \eqref{system linearized around underline U} has a unique solution $U \in L^2([0,T/\epsilon],X^0(\mathbb{R}^d))$ which therefore belongs to $C^0([0,T/\epsilon],X^0(\mathbb{R}^d))$ and satisfies the energy estimates of order $0$ \eqref{energy estimates of order 0}.
\end{mythm}
\begin{proof}
    We consider the Cauchy problem
    \begin{align}\label{Cauchy problem proof existence theorem}
        \begin{cases}
            \partial_t U_{\alpha} + \sum\limits_{j=1}^d A_j(\underline{U})\partial_j J_{\alpha}U_{\alpha} = \epsilon R,\\
            U_{\alpha}|_{t=0} = U_0.
        \end{cases}
    \end{align}
    For $j=1,2$ the operator $A_j(\underline{U})\partial_j J_{\alpha}$ is bounded in $X^0(\mathbb{R}^d)$, so that the Cauchy-Lipschitz theorem gives the existence of solution $U_{\alpha} \in C^0([0,T/\epsilon],X^0(\mathbb{R}^d))$.
    
    The sequence $\{ U_{\alpha}, \alpha \in ]0,1] \}$ is uniformly bounded in $C^0([0,T/\epsilon],X^0(\mathbb{R}^d))$. Indeed, one can do the same as in the proof of Proposition \ref{Energy estimates of order 0 proposition section} to get energy estimates of order $0$ independent of $\alpha$ for the system \eqref{Cauchy problem proof existence theorem}. Moreover through the system \eqref{Cauchy problem proof existence theorem}, we have the boundedness of the sequence $\partial_t U_{\alpha}$ in $C^0([0,T/\epsilon],X^{-1}(\mathbb{R}^d))$.
    
    We also know that $X^0(\mathbb{R}^d)$ and $X^{-1}(\mathbb{R}^d)$ are two reflexive Banach spaces. So thanks to Aubin-Lions theorem, there exists a subsequence, still denoted $U_{\alpha}$ which converges strongly in $L^2([0,T/\epsilon],X^0(\mathbb{R}^d))$ to a function $U \in L^2([0,T/\epsilon],X^0(\mathbb{R}^d))$. We can easily pass to the limit when $\alpha \to 0$ in the equation \eqref{Cauchy problem proof existence theorem}. We get that $U$ is a weak solution of the system \eqref{system linearized around underline U} with $U|_{t=0} = U_0$.
\end{proof}
